Edge modes and symmetry-protected topological states in open quantum systems

Topological order offers possibilities for processing quantum information which can be immune to imperfections. However, the question of its stability out of equilibrium is relevant for experiments, where coupling to an environment is unavoidable. In this work we demonstrate the robustness of certain aspects of $Z_2 \times Z_2$ symmetry-protected topological (SPT) order against a wide class of dissipation channels in the Lindblad and quantum trajectory formalisms of an open quantum system. This is illustrated using the one-dimensional $ZXZ$ cluster Hamiltonian along with Pauli-string jump operators. We show that certain choices of dissipation retaining strong symmetries support a steady-state manifold consisting of two non-local logical qubits, and for Hamiltonian perturbations preserving the global symmetry, states in this manifold remain metastable. In contrast, this metastability is destroyed upon breaking the above-mentioned symmetry. While the localized edge qubits of the cluster Hamiltonian are not conserved by the Lindbladian evolution, they do correspond to weak symmetries and thus retain a memory of their initial state at all times in the quantum trajectories. We utilize this feature to construct protocols to retrieve the quantum information either by monitoring jumps or error mitigation. Our work thus proposes a novel framework to study the dynamics of dissipative SPT phases and opens the possibility of engineering entangled states relevant to quantum information processing.

==> 8_discussion.tex <==
In contrast to previous work which characterised markers of topological order in open systems~\cite{PhysRevB.91.165140,PhysRevX.8.011035,bao2023mixedstate,PhysRevResearch.5.023004,deGroot2022symmetryprotected}, we have gone beyond the mixed-state description by investigating the quantum trajectories of pure states. Moreover, while Ref.~\cite{deGroot2022symmetryprotected} shows that strong symmetries allow string order to survive at finite times in mixed states -- as opposed to disappearing immediately after one discrete time step when only weak symmetries are satisfied by the dissipation -- we provide a class of models with a conserved string order parameter. 
We then proceed to study the resulting non-trivial steady state, in particular exploring its possible practical applications as a quantum memory. 
Building on this, we find analogous phenomena in quantum trajectories under the weaker requirement that the dissipation satisfies weak symmetries.
Our results suggest that the presented models can host stationary qubits, even in the presence of dissipation, as a consequence of weak or strong symmetries.

Realizing the practical and fundamental properties of this family of models could possibly be done in a variety of physical settings.
First, recent experiments have achieved SPT phases in cold atoms~\cite{doi:10.1126/science.aav9105,Sompet2022}. Engineered dissipation is also becoming an available experimental resource either for the preparation of desired states or the study of non-equilibrium quantum phenomena~
\cite{Mi2023Apr}. 
Second, three-qubit gates, which are necessary in our theory, have been engineered recently~\cite{Kim2022Jul,Warren2023May} in circuits of superconducting qubits. Coupling to an environment can also be added readily in these settings, and in particular it can be made to possess engineered symmetries to achieve a desired steady-state~\cite{PhysRevA.88.023849,PhysRevA.88.032317,Kapit_2017,PhysRevLett.116.240503}. Importantly, these devices can be monitored to reproduce physics modelled by quantum trajectories~\cite{PhysRevA.77.012112}.
Third, NISQ (Noisy Intermediate Scale Quantum) devices can also host cluster states, as has been demonstrated in Ref.~\cite{PhysRevLett.125.120502}.
This could be used to probe results presented here in practice and further develop our understanding of topological phases in open quantum systems.
